Graph Attention Networks for Anti-Spoofing

The cues needed to detect spoofing attacks against automatic speaker verification are often located in specific spectral sub-bands or temporal segments. Previous works show the potential to learn these using either spectral or temporal self-attention mechanisms but not the relationships between neighbouring sub-bands or segments. This paper reports our use of graph attention networks (GATs) to model these relationships and to improve spoofing detection performance. GATs leverage a self-attention mechanism over graph structured data to model the data manifold and the relationships between nodes. Our graph is constructed from representations produced by a ResNet. Nodes in the graph represent information either in specific sub-bands or temporal segments. Experiments performed on the ASVspoof 2019 logical access database show that our GAT-based model with temporal attention outperforms all of our baseline single systems. Furthermore, GAT-based systems are complementary to a set of existing systems. The fusion of GAT-based models with more conventional countermeasures delivers a 47% relative improvement in performance compared to the best performing single GAT system.

==> tables/update_all_attack_file.tex <==
\begin{table*}[!ht]
	\small
	\centering
	
	\caption{Results in terms of min t-DCF for development (A01-A06) and evaluation (A07-A19) partitions and respective pooled min~t-DCF (P1) and pooled EER (P2). GAT-S: Spectral attention using GAT. 
	GAT-T: Temporal attention using GAT.
	L:High-spectral-resolution LFCC-GMM,
	R:RawNet2 system. }

	\setlength\tabcolsep{1.5pt}
	\begin{tabularx}{\textwidth}{l || *{6}{Y} |YY| *{13}{Y}| YY} % *{24}{c}
		\hline
		
		S &A01&A02&A03&A04&A05&A06&P1&P2&A07&A08&A09&A10&A11&A12&A13&A14&A15&A16&A17&A18 &A19& P1&P2 	\\ 
		\hline\hline
		GAT-S&.000&.000&.000&.000&.000&.000&.000&.00& .000&.012&.000&.009&.005&.007&.024&.009&.007&.000&.504&.158&.000&{\textbf.085}&3.93\\
	
		\hline
		 GAT-T&.000&.000&.000&.000&.000&.000&.000&.00&.000&.013&.000&.009&.005&.007&.016&.013&.018&.000&.657&.158&.000&0.100&4.71\\
		 \hline
		 L&.000&.000&.000&.001&.000&.000&.000&.00&.001&.001&.000&.154&.005&.115&.080&.069&.069&.006&.352&.074&.008&.090 &	\textbf{3.50}\\
		\hline
		R&.030&.020&.015&.043&.036&.042&.036&1.0&.098&.179&.073&.089&.042&.088&.020&.013&.073&.046&.240&.629&.058&.155&5.54\\
	
		\hline
	\end{tabularx}
	\label{Tab: results on dev and eval}
\end{table*}
